A Rate-Quality Model for Learned Video Coding

Learned video coding (LVC) has recently achieved superior coding performance. In this paper, we model the rate-quality (R-Q) relationship for learned video coding by a parametric function. We learn a neural network, termed RQNet, to characterize the relationship between the bitrate and quality level according to video content and coding context. The predicted (R,Q) results are further integrated with those from previously coded frames using the least-squares method to determine the parameters of our R-Q model on-the-fly. Compared to the conventional approaches, our method accurately estimates the R-Q relationship, enabling the online adaptation of model parameters to enhance both flexibility and precision. Experimental results show that our R-Q model achieves significantly smaller bitrate deviations than the baseline method on commonly used datasets with minimal additional complexity.

==> chapters/3_Results.tex <==
\section{Experimental Results}
\label{sec:results}
% \input{chapters/figures/RQNet_pred}
\input{chapters/figures/curve_visualize}
\subsection{Experimental Settings}
\label{ssec:exp_setting}
\textbf{Datasets:} We use Vimeo-90K \cite{vimeo} to train RQNet and the variable-rate MaskCRT. We randomly crop 256$\times$256 patches for training. The test datasets are HEVC Class B \cite{hevcctc} and UVG \cite{uvg}.

\textbf{Evaluation~Methodologies:} \textcolor{blue}{To evaluate the effectiveness of our RQ-LVC, we conduct the evaluation using two approaches:}
\begin{itemize}
    \item \textit{1-step prediciton strategy}: Our pre-processing step encodes an input video frame-by-frame at various quality levels $Q^{target}$ which are randomly chosen from $[10, 30]$, collecting the resulting per-frame bitrates as the target bitrates $R^{target}$. During this process, we also gather the coding context for each video frame. To assess how effectively our scheme meets $R^{target}$, it predicts a quality level $Q^{pred}$ from the logarithmic R-Q model for each input frame according to $R^{target}$ and the coding context collected from the pre-processing step. The input video frame is then re-encoded with $Q^{pred}$ to measure the deviation of the resulting bitrate from $R^{target}$.
    \item \textcolor{blue}{\textit{Rate control-based strategy}: To allocate bit for frame $X_t$, based on the given target bitrate $R_s$ for each video, we first allocate target bitrate $R_{mg}$ for the corresponding miniGOP, which includes a set of $N_m$ frames $\left\{X_{i},X_{i+1},...,X_{t},...,X_{i+N_{m}-1}\right\}$:
    \begin{equation}
    \label{equ:minigop_allocate}
    R_{mg}=\frac{R_{s}\times\left ( N_{coded}+SW \right )-\hat{R_{s}}}{SW} \times N_{m},
    \end{equation}
    where $N_{coded}$ represents the number of frames that have been encoded, $\hat{R_{s}}$ is the total bitrate already consumed by the current encoding sequence and $SW$ refers to the sliding window size which is set to 40 in our implementation. Afterward, the target bitrate $R_t$ for frame $X_t$ is allocated by:
    \begin{equation}
    \label{equ:frame_allocate}
    R_{t}=\frac{R_{mg}-\hat{R}_{mg}}{\sum_{j=t}^{i+N_{m}-1}}\times w_{t},
    \end{equation}
    where $\hat{R}_{mg}$ is the bitrate already consumed by previously coded frame of the current miniGOP, and $w_t$ denotes the rate allocation weight for frame $X_t$. In this work, we set the number of frame in a miniGOP ($N_m$) equal to 4 and the set of weight for frames within a miniGOP is $\left\{1.9,1.6,1.3,1.0 \right\}$.
    }
\end{itemize}

% The experiments are conducted by encoding the first 32 frames of each video sequence in the test datasets. For each frame at time index $t$, we measure $\Delta R_{t}^{RQNet(n)}$ to assess the accuracy of RQNet in predicting the required bitrate and $\Delta R_{t}^{RC}$ to assess that of our RQ-LVC framework in predicting the quality level for rate control, respectively:
% \begin{equation}
% \label{equ:delta_R_RQNet}
% \Delta R_{t}^{RQNet(n)} = \left | \frac{R_{t}^{GT(n)}-R_{t}^{est(n)}}{R_t^{GT(n)}} \right |\times100\%,
% % \vspace{-0.5cm}
% \end{equation}

% \begin{equation}
% \label{equ:delta_R_RC}
% \Delta R_{t}^{RC} = \left | \frac{R_{t}^{target}-R_{t}^{enc}}{R_t^{target}} \right |\times100\%,
% \end{equation}
% where $R_{t}^{GT(n)}$ represents the ground-truth bitrate obtained by encoding the input video frame at $t$ with quality levels $n=10, 17, 43, 60$, respectively, while $R_{t}^{est(n)}$ denotes the corresponding bitrate predicted by RQNet. $R_{t}^{target}$ and $R_{t}^{enc}$ refer to the target bitrate and the bitrate resulting from encoding the video frame with the predicted quality level $Q_{pred}$ using our logarithmic R-Q model. For each video, we report the average per-frame bitrate deviation in percentage terms. Additionally, we present the complexity of the competing methods in terms of kMAC/pixel and model size. 

% We compare our method with the R-Q update mechanism proposed by Li~\emph{et al.}~\cite{LiLiLambda}. In the Full Set implementation, the first P-frame in each video is encoded 64 times to gather 64 (R,Q) pints for estimating the initial $\alpha,\beta$, whereas the Sub Set approach uses only 4 (R,Q) points, corresponding to $Q= 10,17,43, 60$. Additionally, we include a comparison with the un-weighted least-squares method (w/o weight).


% \input{chapters/figures/RQNet_pred}
% \input{chapters/tables/Rate_Control_Fix_QP}
% \input{chapters/tables/Rate_Control_Var_QP}

The experiments are conducted by encoding the first 96 frames of each video sequence in the test datasets. For each frame at time index $t$, we measure $\Delta R_{t}^{RC}$ to assess the accuracy of our RQ-LVC framework in predicting the quality level for rate control:
\begin{equation}
\label{equ:delta_R_RC}
\Delta R_{t}^{RC} = \left | \frac{R_{t}^{target}-R_{t}^{enc}}{R_t^{target}} \right |\times100\%,
\end{equation}
where $R_{t}^{target}$ and $R_{t}^{enc}$ refer to the target bitrate and the bitrate resulting from encoding the video frame with the predicted quality level $Q^{pred}_{t}$ using our logarithmic R-Q model. For each video, we report the average per-frame bitrate deviation in percentage terms. Additionally, we present the complexity of the competing methods in terms of kMAC/pixel and model size. 

\textbf{Baseline Methods:} We adopt the update strategy proposed by Li~\emph{et al.}~\cite{LiLiLambda} as our baseline method for comparison. As suggested in~\cite{LiLiLambda}, the same initial $\alpha_{t=1}$ and $\beta_{t=1}$ are adopted for each test sequence. In our implementation, they are obtained by averaging their corresponding values over the first frames of all sequences in the two datasets. Based on Eq.~\eqref{equ:Q_real}, the quality level $Q^{real}_t$ is derived from the target bitrate $R^{target}_{t}$ and used to encode the current coding frame $X_t$ with MaskCRT, resulting a bitrate of $R^{real}_t$:
\begin{equation}
\label{equ:Q_real}
Q^{real}_t = \alpha_{t} \times \operatorname{ln}(R^{target}_{t}) + \beta_{t}.
\end{equation}
% \begin{equation}
% \label{equ:R_real}
% R^{real_t} = Encode(X_{t}|Q^{real}_t),
% % \vspace*{-.1cm}
% \end{equation}
With $R^{real}_t$, the corresponding quality level $Q^{est}_t$ is estimated as:
\begin{equation}
\label{equ:Q_est}
Q^{est}_t = \alpha_{t} \times \operatorname{ln}(R^{real}_t) + \beta_{t}.
% \vspace*{-.1cm}
\end{equation}
By adopting the Adaptive Least Mean Square method, the model parameters $\alpha, \beta$ are updated iteratively by Eq.~\eqref{equ:alpha_new}  and Eq.~\eqref{equ:beta_new}, respectively:
\begin{align}
\label{equ:alpha_new}
\alpha_{t+1} &= \alpha_t + \mu \times (Q^{real}_t - Q^{est}_t) \times \ln(R^{real}_t), \\ 
\label{equ:beta_new}
\beta_{t+1} &= \beta_t + \eta \times (Q^{real}_t - Q^{est}_t),
\end{align}
where $\mu$ and $\eta$ are the learning rates, which are set to 0.01 in our experiments.
\textcolor{blue}{Besides, we employ the R-Q model and updating mechanism proposed by Liao~\emph{et al.}~\cite{RC_ICASSP} as a competing method. We also compare our proposed method with the approach described in~\cite{rate_fitting}, which utilizes a neural network (RQNet) to predict R-Q points and generate R-Q model predictions without requiring previously coded (R,Q) points.}
\subsection{Experimental Results}

\textbf{Prediction Accuracy of RQNet and Its Complexity:} Table~\ref{tab:RQNet_acc} presents the prediction accuracy of RQNet, expressed as bitrate deviations in percentage terms. On average, RQNet achieves bitrate deviations of 16.87\% and 15.87\% from the target bitrate on the UVG and HEVC-B dataset, respectively. These deviations tend to be more pronounced at higher bitrates.  Table~\ref{tab:complexity} compares its complexity with that of the base codec, MaskCRT. RQNet's kMAC/pixel is seen to be less than one-tenth of that of MaskCRT, and its model size is only a fraction of MaskCRT's.

%The prediction of the $\alpha$ and $\beta$ coefficients can be performed with just four points predicted by RQNet. However, the accuracy of this estimation may be limited. Therefore, additional (R,Q) points from previously coded frames are needed to enhance accuracy.
%presents a feasible solution with very low complexity to collect the set of points (R,Q), eliminating the need to perform the full frame encoding process at various quality levels.
% \input{chapters/tables/compare_weight}
\input{chapters/tables/RQNet_acc}
\input{chapters/tables/complexity}
% \input{chapters/tables/Rate_Control_Var_QP_NewResults}
% \input{chapters/tables/Rate_Control_96F_1step}
% \input{chapters/tables/Rate_Control_96F_FullRC}
\input{chapters/tables/Rate_Control_96F_combine}

\textbf{Rate Control Performance of RQ-LVC:} Table~\ref{tab:Rate_Control_96F_FullRC} evaluates the rate control performance of our RQ-LVC framework. The target bitrates are produced by encoding every input video frame with a randomly chosen quality level. As shown in the table, RQ-LVC consistently achieves significantly smaller bitrate deviations than the baseline method~\cite{LiLiLambda}. This improvement is attributed to the fact that RQ-LVC leverages the (R,Q) points output by RQNet, along with those from previously coded frames, to estimate the model parameters $\alpha,\beta$. In contrast, Li's method relies exclusively on the (R,Q) points from the past frames. Fig.~\ref{fig:curve_visualize} visualizes the  R-Q functions with the predicted $\alpha,\beta$ for frame 16 across various video sequences, alongside the actual (R,Q) points obtained by encoding the video with various quality levels. The R-Q function predicted by our RQ-LVC closely aligns with the actual (R,Q) points, whereas the R-Q functions predicted by Li~\emph{et al.}~\cite{LiLiLambda} or RQNet only exhibit significant deviations from these ground truths. As presented in Table~\ref{tab:complexity}, the additional overhead introduced by RQNet is minimal compared to MaskCRT, the base codec, both in terms of kMAC/pixel and model size. These attributes make RQ-LVC a practical solution for rate control systems, particularly in scenarios where multi-pass methods are infeasible.

%using the (R,Q) points predicted by RQNet in combination with those gathered from previous frames to estimate $\alpha,\beta$ yields effective quality level predictions. 

% It is also shown that using the weighted least-squares method to predict the parameters is more effective than the conventional method without using weight. This is explained by the fact that frames closer to the current frame are more closely related, so a larger weight should be used for these frames and vice versa. 
% However, in most cases, our proposed method does not perform as well as the approach by Li~\emph{et al.}~\cite{LiLiLambda}, as in the initial frames, our data come primarily from RQNet, whereas Li's method utilizes actual (R,Q) points to initialize $\alpha$ and $\beta$.

\textbf{RQNet Only:} From Table~\ref{tab:Rate_Control_96F_FullRC} and Fig.~\ref{fig:curve_visualize}, it is also evident that using only the (R,Q) points from RQNet (i.e. RQNet Only) to estimate the model parameters is insufficient. As previously analyzed, these predicted (R,Q) points may not always be dependable, especially at higher rates. It is beneficial to leverage also the (R,Q) points from previously coded frames.

\input{chapters/figures/per_frame_rate_dev}
\input{chapters/figures/per_frame_psnr_rate}
%We evaluate the effectiveness of the proposed parameter estimation mechanism using the least-squares approach by comparing our RQ-LVC with a baseline that directly adopts the $\alpha$ and $\beta$ values derived from four points predicted by RQNet without leveraging previously coded information.
%The results indicate that only relying on the prediction of RQNet to fit with R-Q model does not present good performance. In contrast, incorporating the information of the encoded frames combined with the least-squares method to update the model parameters significantly improves accuracy and overall performance.

% \textbf{Impact of the Weighting Strategies: }
% Experimental results with different weighting strategies in the right part of Table~\ref{tab:Rate_Control_Var_QP_NewResults} clearly show that these strategies impact the prediction effectiveness of RQ-LVC. Most videos achieve the best results with linear weighting function, indicating that the current frame should not rely too much on newly generated data points (as in the logarithmic function) or retain excessive information from distant frames (as in the exponential function). Moreover, to evaluate the impact of different weighting methods on the points predicted by RQNet, we conducted experiments with various weighting models, including $\rho\in\left\{ 1/4,1/2,1,2,4\right\}$ and report the results in Table~\ref{tab:compare_weight}. It can be observed that the points predicted by RQNet should be assigned lower weights and contribute less to the model.

% \textbf{Comparison with baseline: }The first column in Table~\ref{tab:Rate_Control_Var_QP_NewResults} displays the bitrate error when applying Li's method~\cite{LiLiLambda} to update the model parameter during the encoding process. We can find that our approach significantly outperforms this competing approach. It can be explained that RQ-LVC leverages a neural network to exploit both the information from the current frame and the information from previously encoded frames, while Li's method solely relies on past information without utilizing any data from the current encoded frame.
% This is because RQNet does not accurately predict the bitrate in the high-rate area. 

% \input{chapters/tables/Rate_Control_Fix_QP}
% \input{chapters/tables/Rate_Control_Var_QP}
% \input{chapters/tables/compare_weight}

% \textbf{Complexity Analysis:} Table~\ref{tab:complexity} outlines the computational complexity of RQNet and RQ-LVC. The additional overhead introduced by RQNet is minimal compared to MaskCRT, the base codec, both in terms of kMAC/pixel and model size. These attributes make RQ-LVC a viable solution for practical rate control systems where multi-pass methods are infeasible.

% The results show that RQ-LVC significantly reduces computational cost (kMAC/pixel) compared to the baseline method while maintaining acceptable rate control accuracy. Additionally, the increase in model size is negligible, as RQNet is considerably simpler than the baseline video encoder. These advantages make RQ-LVC a viable solution for practical rate control systems.
%Meanwhile, the increase in model size is negligible. This efficiency comes from the proposed RQNet, which demonstrates high performance with minimal computational complexity compared to the video encoder.


% \input{chapters/figures/deviation}
% \input{chapters/tables/baseline_vs_proposed}
% \input{chapters/tables/simple_vs_complex}
% \input{chapters/tables/complexity}

==> chapters/figures/RQNet_pred.tex <==
\begin{figure*}[t!]
    \begin{center}
    % \vspace{-1.0em}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/RQNet_prediction/RQNet_Prediction_Beauty.png}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/RQNet_prediction/RQNet_Prediction_Jockey.png}
    \end{subfigure}
    \begin{subfigure}{0.32\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/RQNet_prediction/RQNet_Prediction_BasketballDrive.png}
    \end{subfigure}
    \vspace{-0.1em}
    \caption{The predicted R-Q functions for the first P-frames (Predict) versus their ground truths (GT).}
    \label{fig:RQNet_pred}
    \end{center}
    \vspace{-1.5em}
\end{figure*}

==> chapters/figures/deviation.tex <==
\begin{figure*}[h]
    \begin{center}
    \vspace{-1.0em}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/Baseline_vs_Simple_vs_Compex_Log_BasketballDrive.png}
        % \caption{\centering HEVC Class B}
        \label{fig:Log_BasketballDrive}
        \vspace{-0.5cm}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/Baseline_vs_Simple_vs_Compex_Linear_BasketballDrive.png}
        % \caption{\centering UVG}
        \label{fig:Linear_BasketballDrive}
        \vspace{-0.5cm}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/Baseline_vs_Simple_vs_Compex_Exp_BasketballDrive.png}
        % \caption{\centering MCL-JCV}
        \label{fig:Exp_BasketballDrive}
        \vspace{-0.5cm}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/Baseline_vs_Simple_vs_Compex_Log_HoneyBee.png}
        \label{fig:Log_HoneyBee}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/Baseline_vs_Simple_vs_Compex_Linear_HoneyBee.png}
        \label{fig:Linear_HoneyBee}
    \end{subfigure}
    \begin{subfigure}{0.3\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/Baseline_vs_Simple_vs_Compex_Exp_HoneyBee.png}
        \label{fig:Exp_HoneyBee}
    \end{subfigure}
    \vspace{-0.6cm}
    \caption{The per frame $\Delta R$ of proposed method and baseline method.}
    \label{fig:deviation}
    \end{center}
    \vspace*{-0.7cm}
\end{figure*}

==> chapters/figures/per_frame_psnr_rate.tex <==
% \begin{figure}[t!]
%     \begin{center}
%     \begin{subfigure}{\linewidth}
%         \centering
%         \includegraphics[width=0.85\linewidth]{figures/Per_Rate/QP40/ReadySteadyGo.png}
%     \end{subfigure}
%     \begin{subfigure}{\linewidth}
%     \vspace{0.5em}
%         \centering
%         \includegraphics[width=0.85\linewidth]{figures/Per_Rate/QP40/ParkScene.png}
%         % \label{fig:honey_scale}
%         % \caption{ }
%     \end{subfigure}
%     %\vspace{-3em}
%     \caption{Bitrate and PSNR profiles for ReadySteadyGo and ParkScene.}
%     \label{fig:per_frame_rate_psnr}
%     \end{center}
%     %\vspace{-2.5em}
% \end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.9\linewidth]{figures/Per_Rate/QP40/Cactus.png}
    %\vspace{-3em}
\caption{Bitrate and PSNR profile for Cactus sequence.}
\label{fig:per_frame_rate_psnr}
\vspace{-0.5cm}
\end{figure}

==> chapters/tables/RQNet_Complexity.tex <==
\begin{table}[t!]
\centering
\normalsize
\caption{Complexity of RQNet}
\begin{tabular}{cccc}
\hline
{Model} & {kMAC/pixel} & {Model Size} \\ \hline
MaskCRT        & 2960             & 62.63M             \\
RQNet          & 255              
& 0.764M             \\ \hline
\end{tabular}
\label{tab:RQNet_complexity}
\vspace{-0.5em}
\end{table}

==> chapters/tables/Rate_Control_96F_1step.tex <==
\begin{table*}[t]
\centering
% \footnotesize
\small
\setlength{\tabcolsep}{5pt}
\caption{Bitrate deviations ($\Delta R^{RC}$) of RQ-LVC in percentage terms, with a randomly selected quality level for each video frame.}
\begin{tabular}{ccccccc}
\hline
Dataset                 & Sequence         & Li             & ICASSP'24      & \begin{tabular}[c]{@{}c@{}}RQ-LVC - \\ RQNet Only\end{tabular} & \begin{tabular}[c]{@{}c@{}}RQ-LVC - \\ w/o RQNet\end{tabular} & RQ-LVC                 \\ \hline
\multirow{8}{*}{UVG}    & Beauty           & 12.92          & 10.78          & 3.14                                                           & 4.22                                                          & \textbf{0.96}          \\
                        & Bosphorus        & 10.84          & \textbf{3.23}  & 38.44                                                          & {\ul 5.32}                                                    & 14.17                  \\
                        & HoneyBee         & 21.63          & 51.47          & \textbf{11.30}                                                 & 42.61                                                         & {\ul 20.71}            \\
                        & Jockey           & 16.6           & 8.40           & 11.48                                                          & {\ul 0.77}                                                    & \textbf{0.20}          \\
                        & ReadySteadyGo    & {\ul 1.85}     & 7.66           & \textbf{0.57}                                                  & 5.64                                                          & 8.16                   \\
                        & ShakeNDry        & 64.45          & \textbf{5.25}  & 14.70                                                          & 14.20                                                         & {\ul 5.60}             \\
                        & YachtRide        & 32.00          & 8.38           & 11.12                                                          & 8.33                                                          & \textbf{4.29}          \\
                        & \textit{Average} & \textit{22.90} & \textit{13.60} & \textit{12.96}                                                 & {\ul 11.58}                                                   & \textit{\textbf{7.73}} \\ \hline
\multirow{6}{*}{HEVC-B} & BasketballDrive  & 12.55          & 8.19           & 5.39                                                           & {\ul 5.05}                                                    & \textbf{0.50}          \\
                        & BQTerrace        & 83.84          & \textbf{7.19}  & 16.47                                                          & 24.65                                                         & {\ul 7.43}             \\
                        & Cactus           & 27.24          & 8.06           & \textbf{1.87}                                                  & 7.49                                                          & {\ul 5.74}             \\
                        & Kimono1          & 11.02          & 8.52           & 5.70                                                           & {\ul 4.26}                                                    & \textbf{2.41}          \\
                        & ParkScene        & 38.28          & 7.07           & \textbf{5.48}                                                  & 11.60                                                         & {\ul 5.74}             \\
                        & \textit{Average} & \textit{34.59} & \textit{7.81}  & {\ul \textit{6.98}}                                            & \textit{10.61}                                                & \textit{\textbf{4.36}} \\ \hline
\end{tabular}
\label{tab:Rate_Control_96F_1step}
% \vspace{-0.5em}
\vspace{0.1em}
\end{table*}

==> chapters/tables/Rate_Control_96F_combine.tex <==
\begin{table*}[t]
\centering
\footnotesize
% \small
\setlength{\tabcolsep}{2.3pt}
\caption{Bitrate deviations ($\Delta R^{RC}$) of RQ-LVC in percentage terms, with rate control process.}
\fontsize{7.5}{9}\selectfont
\begin{tabular}{cc|ccccc|ccccc}
\hline
\multirow{2}{*}{Dataset}                                                & \multirow{2}{*}{Sequence} & \multicolumn{5}{c|}{1-step prediction}                                                                                                                                                                                                                                                  & \multicolumn{5}{c}{Rate control}                                                                                                                                                                                                                                                        \\ \cline{3-12} 
                                                                        &                           & \begin{tabular}[c]{@{}c@{}}TIP'14\\\cite{LiLiLambda}\end{tabular} & \begin{tabular}[c]{@{}c@{}}ICASSP'24\\\cite{RC_ICASSP}\end{tabular} & \begin{tabular}[c]{@{}c@{}}RQNet Only\\(DCC'25~\cite{rate_fitting})\end{tabular} & \begin{tabular}[c]{@{}c@{}}RQ-LVC - \\ w/o RQNet\end{tabular} & RQ-LVC                 & \begin{tabular}[c]{@{}c@{}}TIP'14\\\cite{LiLiLambda}\end{tabular} & \begin{tabular}[c]{@{}c@{}}ICASSP'24\\\cite{RC_ICASSP}\end{tabular} & \begin{tabular}[c]{@{}c@{}}RQNet Only\\(DCC'25~\cite{rate_fitting})\end{tabular} & \begin{tabular}[c]{@{}c@{}}RQ-LVC - \\ w/o RQNet\end{tabular} & RQ-LVC                 \\ \hline
\multirow{8}{*}{UVG}                                                    & Beauty                    & 12.92                                                        & 10.78                                                          & 3.14                                                           & 4.22                                                          & \textbf{0.96}          & 2.15                                                         & 3.47                                                           & 6.47                                                           & \textbf{1.70}                                                 & {\ul 2.07}                   \\
                                                                        & Bosphorus                 & 10.84                                                        & \textbf{3.23}                                                  & 38.44                                                          & {\ul 5.32}                                                    & 14.17                  & 4.38                                                         & 1.41                                                           & 7.50                                                           & {\ul 0.82}                                                    & \textbf{0.46}          \\
                                                                        & HoneyBee                  & 21.63                                                        & 51.47                                                          & \textbf{11.30}                                                 & 42.61                                                         & {\ul 20.71}            & 6.63                                                         & 34.09                                                          & {\ul 2.88}                                                     & 13.25                                                         & \textbf{2.23}          \\
                                                                        & Jockey                    & 16.6                                                         & 8.40                                                           & 11.48                                                          & {\ul 0.77}                                                    & \textbf{0.20}          & 4.99                                                         & 1.71                                                           & 4.18                                                           & \textbf{0.74}                                                 & {\ul 1.58}             \\
                                                                        & ReadySteadyGo             & {\ul 1.85}                                                   & 7.66                                                           & \textbf{0.57}                                                  & 5.64                                                          & 8.16                   & 2.96                                                         & 1.97                                                           & 4.47                                                           & {\ul 1.15}                                                    & \textbf{0.84}          \\
                                                                        & ShakeNDry                 & 64.45                                                        & \textbf{5.25}                                                  & 14.70                                                          & 14.20                                                         & {\ul 5.60}             & 5.97                                                         & 2.65                                                           & 2.21                                                           & {\ul 1.31}                                                    & \textbf{0.88}          \\
                                                                        & YachtRide                 & 32.00                                                        & 8.38                                                           & 11.12                                                          & 8.33                                                          & \textbf{4.29}          & 3.21                                                         & 2.27                                                           & {\ul 1.09}                                                     & 1.38                                                          & \textbf{1.04}          \\
                                                                        & \textit{Average}          & \textit{22.90}                                               & \textit{13.60}                                                 & \textit{12.96}                                                 & {\ul 11.58}                                                   & \textit{\textbf{7.73}} & \textit{4.33}                                                & \textit{6.80}                                                  & \textit{4.11}                                                  & {\ul 2.90}                                                    & \textit{\textbf{1.30}} \\ \hline
\multirow{6}{*}{\begin{tabular}[c]{@{}c@{}}HEVC\\ Class B\end{tabular}} & BasketballDrive           & 12.55                                                        & 8.19                                                           & 5.39                                                           & {\ul 5.05}                                                    & \textbf{0.50}          & 2.24                                                         & 3.65                                                           & {\ul 1.77}                                                     & 2.21                                                          & \textbf{1.63}          \\
                                                                        & BQTerrace                 & 83.84                                                        & \textbf{7.19}                                                  & 16.47                                                          & 24.65                                                         & {\ul 7.43}             & 11.69                                                        & 1.96                                                           & {\ul 1.10}                                                     & 3.58                                                          & \textbf{0.88}          \\
                                                                        & Cactus                    & 27.24                                                        & 8.06                                                           & \textbf{1.87}                                                  & 7.49                                                          & {\ul 5.74}             & 1.08                                                         & 2.72                                                           & 2.27                                                           & {\ul 1.88}                                                    & \textbf{0.57}          \\
                                                                        & Kimono1                   & 11.02                                                        & 8.52                                                           & 5.70                                                           & {\ul 4.26}                                                    & \textbf{2.41}          & 2.12                                                         & 2.52                                                           & 2.60                                                           & {\ul 0.81}                                                    & \textbf{0.40}          \\
                                                                        & ParkScene                 & 38.28                                                        & 7.07                                                           & \textbf{5.48}                                                  & 11.60                                                         & {\ul 5.74}             & 0.96                                                         & 2.53                                                           & 2.04                                                           & {\ul 1.45}                                                    & \textbf{0.59}          \\
                                                                        & \textit{Average}          & \textit{34.59}                                               & \textit{7.81}                                                  & {\ul \textit{6.98}}                                            & \textit{10.61}                                                & \textit{\textbf{4.36}} & \textit{3.62}                                                & \textit{2.67}                                                  & {\ul \textit{1.96}}                                            & \textit{1.99}                                                 & \textit{\textbf{0.81}} \\ \hline
\end{tabular}
\label{tab:Rate_Control_96F_FullRC}
% \vspace{-0.5em}
\vspace{0.1em}
\end{table*}

==> chapters/tables/Rate_Control_Fix_QP.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
% \normalsize
\scriptsize
\setlength{\tabcolsep}{5pt}
\caption{Bitrate error ($\Delta R^{RC}$) of RQ-LVC from a rate control perspective, with a fixed quality level for each frame.}
\begin{tabular}{>{\centering\arraybackslash}p{0.75cm} >{\centering\arraybackslash}p{1.35cm}>{\centering\arraybackslash}p{0.7cm}>{\centering\arraybackslash}p{0.7cm}>{\centering\arraybackslash}p{0.62cm}>{\centering\arraybackslash}p{0.62cm}>{\centering\arraybackslash}p{0.62cm}>{\centering\arraybackslash}p{0.48cm}}
\hline
\multirow{3}{*}{Dataset} & \multirow{3}{*}{Sequence} & \multirow{3}{*}{{\begin{tabular}[c]{@{}c@{}}Li~\emph{et al.}\\Full Set\end{tabular}}} & \multirow{3}{*}{{\begin{tabular}[c]{@{}c@{}}Li~\emph{et al.}\\Sub Set\end{tabular}}} & \multicolumn{4}{c}{RQ-LVC}                                                                                                                      \\ \cline{5-8} 
                                  &                                    &                                                                                                                     &                                                                                                                    & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}w/o\\ weight\end{tabular}} & \multicolumn{3}{c}{w/ weight}                                  \\ \cline{6-8} 
                                  &                                    &                                                                                                                     &                                                                                                                    &                                                                                & Log           & Linear        & Exp          \\ \hline
\multirow{8}{*}{UVG}              & Beauty                             & 2.78                                                                                                                & 2.73                                                                                                               & 8.24                                                                           & 7.41                   & 6.35                   & 4.74                   \\
                                  & Bosphorus                          & 2.86                                                                                                                & 4.32                                                                                                               & 7.28                                                                           & 6.45                   & 5.68                   & 6.33                   \\
                                  & HoneyBee                           & 4.82                                                                                                                & 3.53                                                                                                               & 14.44                                                                          & 13.77                  & 11.78                  & 9.61                   \\
                                  & Jockey                             & 2.36                                                                                                                & 2.00                                                                                                               & 4.06                                                                           & 3.71                   & 4.01                   & 5.42                   \\
                                  & ReadySteadyGo                      & 2.77                                                                                                                & 3.12                                                                                                               & 13.85                                                                          & 10.78                  & 8.47                   & 6.56                   \\
                                  & ShakeNDry                          & 0.96                                                                                                                & 0.84                                                                                                               & 6.60                                                                           & 5.86                   & 5.50                   & 8.41                   \\
                                  & YachtRide                          & 2.05                                                                                                                & 2.58                                                                                                               & 8.10                                                                           & 7.80                   & 7.17                   & 8.47                   \\
                                  & \textit{Average}                   & \textit{2.66}                                                                                                       & \textit{2.73}                                                                                                      & \textit{8.94}                                                                  & \textit{7.97}          & \textit{6.99}          & \textit{7.08}          \\ \hline
\multirow{6}{*}{HEVC-B}           & BasketballDrive                    & 2.51                                                                                                                & 2.55                                                                                                               & 6.31                                                                           & 6.53                   & 6.58                   & 7.19                   \\
                                  & BQTerrace                          & 3.43                                                                                                                & 3.51                                                                                                               & 7.06                                                                           & 6.98                   & 6.33                   & 6.40                   \\
                                  & Cactus                             & 4.35                                                                                                                & 4.45                                                                                                               & 13.08                                                                          & 12.66                  & 11.43                  & 9.70                   \\
                                  & Kimono1                            & 1.49                                                                                                                & 1.56                                                                                                               & 3.75                                                                           & 3.66                   & 3.53                   & 3.56                   \\
                                  & ParkScene                          & 3.94                                                                                                                & 3.63                                                                                                               & 4.75                                                                           & 4.13                   & 3.80                   & 4.16                   \\
                                  & \textit{Average}                   & \textit{3.14}                                                                                                       & \textit{3.14}                                                                                                      & 6.99                                                                           & \textit{6.79}          & \textit{6.33}          & \textit{6.20}          \\ \hline
\multicolumn{2}{c}{\textit{\textbf{Average}}}                          & \textit{\textbf{2.86}}                                                                                              & \textit{\textbf{2.90}}                                                                                             & \textit{\textbf{8.13}}                                                         & \textit{\textbf{7.48}} & \textit{\textbf{6.72}} & \textit{\textbf{6.71}} \\ \hline
\end{tabular}
\label{tab:Rate_Control_Fix_QP}
\vspace{-0.5em}
\end{table}

==> chapters/tables/Rate_Control_Var_QP.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
% \normalsize
\scriptsize
\setlength{\tabcolsep}{5pt}
\caption{Bitrate error ($\Delta R^{RC}$) of RQ-LVC from a rate control perspective, with random quality level selection.}
\begin{tabular}{>{\centering\arraybackslash}p{0.75cm} >{\centering\arraybackslash}p{1.35cm}>{\centering\arraybackslash}p{0.7cm}>{\centering\arraybackslash}p{0.7cm}>{\centering\arraybackslash}p{0.62cm}>{\centering\arraybackslash}p{0.62cm}>{\centering\arraybackslash}p{0.62cm}>{\centering\arraybackslash}p{0.6cm}}
\hline
\multirow{3}{*}{Dataset} & \multirow{3}{*}{Sequence} & \multirow{3}{*}{{\begin{tabular}[c]{@{}c@{}}Li~\emph{et al.}\\ Full Set\end{tabular}}} & \multirow{3}{*}{{\begin{tabular}[c]{@{}c@{}}Li~\emph{et al.}\\ Sub Set\end{tabular}}} & \multicolumn{4}{c}{{RQ-LVC}}                                                                                                                          \\ \cline{5-8} 
                                  &                                    &                                                                                                                     &                                                                                                                    & \multirow{2}{*}{{\begin{tabular}[c]{@{}c@{}}w/o\\ weight\end{tabular}}} & \multicolumn{3}{c}{{w/ weight}}                                      \\ \cline{6-8} 
                                  &                                    &                                                                                                                     &                                                                                                                    &                                                                                & {Log}            & {Linear}         & {Exp}            \\ \hline
\multirow{8}{*}{UVG}              & Beauty                             & 7.19                                                                                                                & 6.95                                                                                                               & 9.02                                                                           & 8.78                    & 7.67                    & 7.21                    \\
                                  & Bosphorus                          & 26.57                                                                                                               & 30.71                                                                                                              & 23.41                                                                          & 22.71                   & 21.71                   & 27.20                   \\
                                  & HoneyBee                           & 12.32                                                                                                               & 12.71                                                                                                              & 14.85                                                                          & 14.16                   & 14.00                   & 14.70                   \\
                                  & Jockey                             & 5.62                                                                                                                & 5.38                                                                                                               & 5.93                                                                           & 6.33                    & 6.28                    & 7.83                    \\
                                  & ReadySteadyGo                      & 8.57                                                                                                                & 8.71                                                                                                               & 15.21                                                                          & 15.47                   & 13.21                   & 12.06                   \\
                                  & ShakeNDry                          & 2.08                                                                                                                & 2.04                                                                                                               & 5.57                                                                           & 4.35                    & 5.14                    & 7.83                    \\
                                  & YachtRide                          & 7.65                                                                                                                & 8.09                                                                                                               & 9.56                                                                           & 8.49                    & 8.62                    & 9.50                    \\
                                  & \textit{Average}                   & \textit{10.00}                                                                                                      & \textit{10.66}                                                                                                     & \textit{11.94}                                                                 & \textit{11.47}          & \textit{10.95}          & \textit{12.33}          \\ \hline
\multirow{6}{*}{HEVC-B}           & BasketballDrive                    & 6.34                                                                                                                & 6.57                                                                                                               & 9.43                                                                           & 9.05                    & 8.89                    & 8.74                    \\
                                  & BQTerrace                          & 15.41                                                                                                               & 19.79                                                                                                              & 8.32                                                                           & 7.90                    & 9.58                    & 14.20                   \\
                                  & Cactus                             & 12.21                                                                                                               & 13.85                                                                                                              & 13.13                                                                          & 12.96                   & 12.60                   & 12.68                   \\
                                  & Kimono1                            & 4.24                                                                                                                & 4.31                                                                                                               & 6.44                                                                           & 6.61                    & 6.16                    & 5.64                    \\
                                  & ParkScene                          & 14.79                                                                                                               & 15.24                                                                                                              & 9.88                                                                           & 9.27                    & 10.59                   & 12.96                   \\
                                  & \textit{Average}                   & \textit{10.60}                                                                                                      & \textit{11.95}                                                                                                     & \textit{9.44}                                                                  & \textit{9.16}           & \textit{9.56}           & \textit{10.84}          \\ \hline
\multicolumn{2}{c}{\textbf{Average}}                                   & \textit{\textbf{10.25}}                                                                                             & \textit{\textbf{11.20}}                                                                                            & \textit{\textbf{10.90}}                                                        & \textit{\textbf{10.51}} & \textit{\textbf{10.37}} & \textit{\textbf{11.71}} \\ \hline
\end{tabular}
\label{tab:Rate_Control_Var_QP}
% \vspace{-0.5em}
\vspace{-0.1em}
\end{table}

==> chapters/tables/Rate_Control_Var_QP_NewResults.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\footnotesize
% \scriptsize
\setlength{\tabcolsep}{5pt}
\caption{Bitrate deviations ($\Delta R^{RC}$) of RQ-LVC in percentage terms, with a randomly selected quality level for each video frame.}
\begin{tabular}{ccccc}
\hline
Dataset                 & Sequence         & \begin{tabular}[c]{@{}c@{}}Li~\emph{et al.}\\ ~\cite{LiLiLambda}\end{tabular} & \begin{tabular}[c]{@{}c@{}}RQNet\\ Only\end{tabular} & RQ-LVC         \\ \hline
\multirow{8}{*}{UVG}    & Beauty           & 7.6                                                                                                             & 6.19                                                 & 9.02           \\
                        & Bosphorus        & 46.94                                                                                                           & 47.36                                                & 23.41          \\
                        & HoneyBee         & 45.4                                                                                                            & 16.16                                                & 14.85          \\
                        & Jockey           & 8.41                                                                                                            & 13.96                                                & 5.93           \\
                        & ReadySteadyGo    & 11.29                                                                                                           & 12.41                                                & 15.21          \\
                        & ShakeNDry        & 10.44                                                                                                           & 14.16                                                & 5.57           \\
                        & YachtRide        & 7.16                                                                                                            & 11.51                                                & 9.56           \\
                        & \textit{Average} & 19.61                                                                                                           & \textit{17.39}                                       & \textit{11.94} \\ \hline
\multirow{6}{*}{HEVC-B} & BasketballDrive  & 5.57                                                                                                            & 10.60                                                 & 9.43           \\
                        & BQTerrace        & 34.03                                                                                                           & 33.02                                                & 8.32           \\
                        & Cactus           & 13.31                                                                                                           & 17.22                                                & 13.13          \\
                        & Kimono1          & 7.13                                                                                                            & 6.89                                                 & 6.44           \\
                        & ParkScene        & 21.14                                                                                                           & 20.7                                                 & 9.88           \\
                        & \textit{Average} & 16.24                                                                                                           & \textit{17.69}                                       & \textit{9.44}  \\ \hline
\end{tabular}
\label{tab:Rate_Control_Var_QP_NewResults}
% \vspace{-0.5em}
\vspace{0.1em}
\end{table}

==> chapters/tables/baseline_vs_proposed.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[h]
\caption{$\Delta R$ comparison of the proposed method and Baseline method. The smaller $\Delta R$ the better.}
\footnotesize
\centering

\begin{tabular}{cccccc|cccc}
\hline
                          &                            & \multicolumn{4}{c|}{Baseline}                                                                                                                                                                                                              & \multicolumn{4}{c}{Proposed}                                                                                                                                                                                                             \\ \cline{3-10} 
\multirow{-2}{*}{Dataset} & \multirow{-2}{*}{Sequence} & \begin{tabular}[c]{@{}c@{}}Normal\\ LMS\end{tabular} & \begin{tabular}[c]{@{}c@{}}Weighted, \\ Log\end{tabular} & \begin{tabular}[c]{@{}c@{}}Weighted, \\ Linear\end{tabular} & \begin{tabular}[c]{@{}c@{}}Weighted, \\ Exp\end{tabular} & \begin{tabular}[c]{@{}c@{}}Normal\\ LMS\end{tabular} & \begin{tabular}[c]{@{}c@{}}Weighted, \\ Log\end{tabular} & \begin{tabular}[c]{@{}c@{}}Weighted, \\ Linear\end{tabular} & \begin{tabular}[c]{@{}c@{}}Weighted, \\ Exp\end{tabular} \\ \hline
                          & Beauty                     & 0.034                        						  & 0.084                                                    & 0.075                                                       & 0.086                                                    & 0.079                        						 & 0.092                                                    & 0.090                                                       & 0.096                                                    \\
                          & Bosphorus                  & 0.15                                                 & 0.114                                                    & 0.106                                                       & 0.101                                      			  & 0.129                                                & 0.149                                                    & 0.200                                                       & 0.203                                                    \\
                          & HoneyBee                   & 0.175                                                & 0.170                                                    & 0.153                                                       & 0.161                                                    & 0.167                                                & 0.148                                                    & 0.143                                                       & 0.145                                                    \\
                          & Jockey                     & 0.043                                                & 0.040                                                    & 0.040                                                       & 0.040                                                    & 0.111                                                & 0.074                                                    & 0.066                                                       & 0.075                                                    \\
                          & ReadySteadyGo              & 0.085                                                & 0.094                                                    & 0.091                                                       & 0.115                                                    & 0.096                                                & 0.157                                                    & 0.160                                                       & 0.164                                                    \\
                          & ShakeNDry                  & 0.010                                                & 0.039                                                    & 0.034                                                       & 0.043                                                    & 0.045                                                & 0.038                                                    & 0.036                                                       & 0.039                                                    \\
						  & YachtRide                  & 0.048                                                & 0.075                                                    & 0.067                                                       & 0.071                                                    & 0.073                                                & 0.078                                                    & 0.073                                                       & 0.073                                                    \\ 
\multirow{-8}{*}{UVG}     & \textit{Average}                    & \textit{0.078}                                                & \textit{0.088}                                                    & \textit{0.081}                                                       & \textit{0.088}                                                    & \textit{0.100}                                                & \textit{0.105}                                                    & \textit{0.110}                                                       & \textit{0.114 }                                                   \\ \hline

                          & BasketballDrive            & 0.077                                                & 0.071                                                    & 0.072                                                       & 0.071                                                    & 0.085                                                & 0.073                                                    & 0.074                                                       & 0.074                                                    \\
                          & BQTerrace                  & 0.054                                                & 0.050                                                    & 0.049                                                       & 0.052                                                    & 0.199                                                & 0.052                                                    & 0.051                                                       & 0.051                                                    \\
                          & Cactus                     & 0.084                                                & 0.122                                                    & 0.118                                                       & 0.121                                                    & 0.196                                                & 0.121                                                    & 0.117                                                       & 0.119                                                    \\
                          & Kimono1                    & 0.029                                                & 0.047                                                    & 0.046                                                       & 0.044                                                    & 0.067                                                & 0.049                                                    & 0.050                                                       & 0.053                                                    \\
						  & ParkScene                  & 0.136                                                & 0.078                                                    & 0.074                                                       & 0.079                                                    & 0.055                                                & 0.089                                                    & 0.082                                                       & 0.085                                                    \\ 
\multirow{-6}{*}{HEVC-B}  & \textit{Average}                    & \textit{0.076}                                                & \textit{0.074}                                                    & \textit{0.072}                                                       & \textit{0.073}                                                    & \textit{0.120}                                                & \textit{0.077}                                                    & \textit{0.075}                                                       & \textit{0.076}                                                    \\ \hline

\end{tabular}
\label{tab:baseline_propose}
\vspace{-.25cm}
\end{table*}

==> chapters/tables/compare_weight.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
\centering
\footnotesize
\caption{Comparison of different weighting methods for the points predicted by RQNet.}
\begin{tabular}{cccccc}
\hline
\multirow{2}{*}{{Dataset}} & \multicolumn{5}{c}{{$\Delta R^{RC} (\downarrow )$}}                                                                                                                                                           \\ \cline{2-6} 
                                  & \multicolumn{1}{c}{{$\rho$=1/4}} & \multicolumn{1}{c}{{$\rho$=1/2}} & \multicolumn{1}{c}{{$\rho$=1}} & \multicolumn{1}{c}{{$\rho$=2}} & \multicolumn{1}{c}{{$\rho$=4}} \\ \hline
UVG                               & 11.47                                   & 11.37                                   & 11.36                                 & 11.55                                 & 12.23                                 \\
HEVC-B                            & 9.15                                    & 9.24                                    & 9.52                                  & 10.02                                 & 10.65                                 \\ \hline
\textit{\textbf{Average}}         & \textit{\textbf{10.50}}                 & \textit{\textbf{10.48}}                 & \textit{\textbf{10.59}}               & \textit{\textbf{10.92}}               & \textit{\textbf{11.57}}               \\ \hline
\end{tabular}
\label{tab:compare_weight}
% \vspace{-2.5em}
\end{table}





% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[t]
% \scriptsize
% \caption{Comparison between weighting strategy.}
% \begin{tabular}{ccccccc}
% \hline
% \multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Sequence}} & \multicolumn{5}{c}{\textbf{Weighting Function}}                                                                                 \\ \cline{3-7} 
%                                   &                                    & \textbf{t/4}            & \textbf{t/2}            & \textbf{t}              & \textbf{2*t}            & \textbf{4*t}            \\ \hline
% \multirow{8}{*}{UVG}              & Beauty                             & 0.089                   & 0.086                   & 0.083                   & 0.078                   & 0.074                   \\
%                                   & Bosphorus                          & 0.230                   & 0.226                   & 0.224                   & 0.236                   & 0.265                   \\
%                                   & HoneyBeee                          & 0.142                   & 0.143                   & 0.145                   & 0.148                   & 0.149                   \\
%                                   & Jockey                             & 0.060                   & 0.058                   & 0.059                   & 0.064                   & 0.075                   \\
%                                   & ReadSteadyGo                       & 0.151                   & 0.147                   & 0.141                   & 0.130                   & 0.122                   \\
%                                   & ShakeNDry                          & 0.045                   & 0.048                   & 0.052                   & 0.061                   & 0.073                   \\
%                                   & YachtRide                          & 0.086                   & 0.087                   & 0.091                   & 0.095                   & 0.095                   \\
%                                   & \textit{Average}                   & \textit{0.115}          & \textit{0.114}          & \textit{0.114}          & \textit{0.116}          & \textit{0.122}          \\ \hline
% \multirow{6}{*}{HEVC-B}           & BasketballDrive                    & 0.092                   & 0.091                   & 0.09                    & 0.089                   & 0.088                   \\
%                                   & BQTerrace                          & 0.079                   & 0.082                   & 0.091                   & 0.107                   & 0.132                   \\
%                                   & Cactus                             & 0.129                   & 0.129                   & 0.13                    & 0.132                   & 0.132                   \\
%                                   & Kimono1                            & 0.065                   & 0.064                   & 0.063                   & 0.061                   & 0.057                   \\
%                                   & ParkScene                          & 0.093                   & 0.096                   & 0.102                   & 0.112                   & 0.124                   \\
%                                   & \textit{Average}                   & \textit{0.092}          & \textit{0.092}          & \textit{0.095}          & \textit{0.100}          & \textit{0.107}          \\ \hline
% \multicolumn{2}{c}{\textit{\textbf{Average}}}                          & \textit{\textbf{0.105}} & \textit{\textbf{0.105}} & \textit{\textbf{0.106}} & \textit{\textbf{0.109}} & \textit{\textbf{0.116}} \\ \hline
% \end{tabular}
% \label{tab:compare_weight}
% % \vspace{-2.5em}
% \end{table}

==> chapters/tables/complexity.tex <==
\begin{table}[t!]
\centering
\footnotesize
\caption{Complexity analysis of RQ-LVC.}
\begin{tabular}{ccc}
\hline
Model   & kMAC/pixel & Model Size \\ \hline
RQNet   & 255     & 0.76 M     \\
MaskCRT & 2960    & 62.63 M     \\
RQ-LVC  & 3215    & 63.39 M      \\ \hline
\end{tabular}
\label{tab:complexity}
% \vspace{-0.5em}
\end{table}

==> chapters/tables/simple_vs_complex.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[h!]
\caption{$\Delta R$ comparison of the proposed $Simple$ and $Complex$ implementation version. The smaller $\Delta R$ the better.}
\centering
\footnotesize
\begin{tabular}{ccccc|ccc}
\hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Sequence} & \multicolumn{3}{c|}{Simple}                                                                                                                                                        & \multicolumn{3}{c}{Complex}                                                                                                                                                       \\ \cline{3-8} 
                         &                           & \begin{tabular}[c]{@{}c@{}}Weighted, \\ Log\end{tabular} & \begin{tabular}[c]{@{}c@{}}Weighted, \\ Linear\end{tabular} & \begin{tabular}[c]{@{}c@{}}Weighted, \\ Exp\end{tabular} & \begin{tabular}[c]{@{}c@{}}Weighted, \\ Log\end{tabular} & \begin{tabular}[c]{@{}c@{}}Weighted, \\ Linear\end{tabular} & \begin{tabular}[c]{@{}c@{}}Weighted, \\ Exp\end{tabular} \\ \hline
\multirow{8}{*}{UVG}     & Beauty                    & 0.092                                                    & 0.090                                                       & 0.096                                                    & 0.088                                                    & 0.079                                                       & 0.071                                                    \\
                         & Bosphorus                 & 0.149                                                    & 0.200                                                       & 0.203                                                    & 0.123                                                    & 0.119                                                       & 0.128                                                    \\
                         & HoneyBee                  & 0.148                                                    & 0.143                                                       & 0.145                                                    & 0.147                                                    & 0.142                                                       & 0.135                                                    \\
                         & Jockey                    & 0.074                                                    & 0.066                                                       & 0.075                                                    & 0.050                                                    & 0.050                                                       & 0.069                                                    \\
                         & ReadySteadyGo             & 0.157                                                    & 0.160                                                       & 0.164                                                    & 0.097                                                    & 0.079                                                       & 0.077                                                    \\
                         & ShakeNDry                 & 0.038                                                    & 0.036                                                       & 0.039                                                    & 0.037                                                    & 0.034                                                       & 0.036                                                    \\
                         & YachtRide                 & 0.078                                                    & 0.073                                                       & 0.073                                                    & 0.075                                                    & 0.067                                                       & 0.056                                                    \\ 
                         & \textit{Average}                   & \textit{0.105}                                                    & \textit{0.110}                                                       & \textit{0.114}                                                    & \textit{0.088}                                                    & \textit{0.081}                                                       & \textit{0.082}                                                    \\ \hline

\multirow{6}{*}{HEVC-B}  & BasketballDrive           & 0.073                                                    & 0.074                                                       & 0.074                                                    & 0.071                                                    & 0.073                                                       & 0.070                                                    \\
                         & BQTerrace                 & 0.052                                                    & 0.051                                                       & 0.051                                                    & 0.049                                                    & 0.045                                                       & 0.043                                                    \\
                         & Cactus                    & 0.121                                                    & 0.117                                                       & 0.119                                                    & 0.112                                                    & 0.095                                                       & 0.085                                                    \\
                         & Kimono1                   & 0.049                                                    & 0.050                                                       & 0.053                                                    & 0.049                                                    & 0.053                                                       & 0.055                                                    \\
                         & ParkScene                 & 0.089                                                    & 0.082                                                       & 0.085                                                    & 0.076                                                    & 0.068                                                       & 0.069                                                    \\ 
                         & \textit{Average}                   & \textit{0.077}                                                    & \textit{0.075}                                                       & \textit{0.076}                                                    & \textit{0.071}                                                    & \textit{0.067}                                                       & \textit{0.064 }                                                   \\ \hline

\end{tabular}
\label{tab:simple_vs_complex}
\vspace{-0.5cm}
\end{table*}
